X-ray Redshifts for Obscured Active Galactic Nuclei with AXIS Deep and Intermediate Surveys

This study presents the capabilities of the AXIS telescope in estimating redshifts from X-ray spectra alone (X-ray redshifts, XZs). Through extensive simulations, we establish that AXIS observations enable reliable XZ estimates for more than 5500 obscured Active Galactic Nuclei (AGN) up to redshift $z\sim 6$ in the proposed deep (7 Ms) and intermediate (375 ks) surveys. Notably, at least 1600 of them are expected to be in the Compton-Thick regime ($\log N_H/\mathrm{cm^{-2}}\geq 24$), underscoring the pivotal role of AXIS in sample these elusive objects that continue to be poorly understood. XZs provide an efficient alternative for optical/infrared faint sources, overcoming the need for time-consuming spectroscopy, potential limitations of photometric redshifts, and potential issues related to multi-band counterpart association. This approach will significantly enhance the accuracy of constraints on the X-ray luminosity function and obscured AGN fractions up to high redshift. This White Paper is part of a series commissioned for the AXIS Probe Concept Mission; additional AXIS White Papers can be found at the AXIS website (http://axis.astro.umd.edu) with a mission overview here: arXiv:2311.00780.

==> Definitions/journalnames.tex <==
\DeclareOption{ArXiv}{ 	    \gdef\@journal{ArXiv}	\gdef\@journalshort{ArXiv}	\gdef\@journalfull{ArXiv}	\gdef\@doiabbr{ArXiv}	}
